A Survey on Deep Stereo Matching in the Twenties

Stereo matching is close to hitting a half-century of history, yet witnessed a rapid evolution in the last decade thanks to deep learning. While previous surveys in the late 2010s covered the first stage of this revolution, the last five years of research brought further ground-breaking advancements to the field. This paper aims to fill this gap in a two-fold manner: first, we offer an in-depth examination of the latest developments in deep stereo matching, focusing on the pioneering architectural designs and groundbreaking paradigms that have redefined the field in the 2020s; second, we present a thorough analysis of the critical challenges that have emerged alongside these advances, providing a comprehensive taxonomy of these issues and exploring the state-of-the-art techniques proposed to address them. By reviewing both the architectural innovations and the key challenges, we offer a holistic view of deep stereo matching and highlight the specific areas that require further investigation. To accompany this survey, we maintain a regularly updated project page that catalogs papers on deep stereo matching in our Awesome-Deep-Stereo-Matching (https://github.com/fabiotosi92/Awesome-Deep-Stereo-Matching) repository.

==> chapters/2_datasets.tex <==
\begin{figure*}[t]
    \centering
    \begin{overpic}
    [clip,trim=0cm 3cm 1cm 0cm,width=\linewidth]{images/survey_stereo_synth.pdf}
    \put (10,18.4) {\scalebox{.65}{Virtual KITTI 2 \cite{cabon2020virtual}}}
    \put (29,18.4) {\scalebox{.65}{Dynamic Replica \cite{Karaev_2023_CVPR}}}
    \put (10,1) {\scalebox{.65}{UnrealStereo4K \cite{Tosi2021CVPR_SMD}}}
    \put (32,1) {\scalebox{.65}{IRS \cite{wang2021irs}}}
    \put (52,1) {\scalebox{.65}{CREStereo \cite{li2022practical_CREStereo}}}
    \put (82.5,1) {\scalebox{.65}{Spring \cite{Mehl2023_Spring}}}
    \end{overpic}\vspace{-0.3cm}
    \caption{\textbf{New stereo datasets in the 20s (Synthetic).}}
    \label{fig:synth_dataset}
\end{figure*}

\section{Datasets}
\label{sec:datasets}

In this section, we introduce the most relevant datasets being released in the 20ies. For details about datasets available before, we refer the reader to previous surveys \cite{poggi2021synergies,laga2020survey}.

\subsection{Real-World}

We start by listing those datasets collecting real stereo images and, optionally, ground truth disparity maps acquired by means of active sensors. Fig. \ref{fig:real_datasets} shows an overview of some samples taken from these datasets.

\subsubsection{Passive Stereo Datasets}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Middlebury 2021 Mobile Dataset
% https://vision.middlebury.edu/stereo/data/scenes2021/
\textbf{Middlebury 2021} \cite{scharstein2014high}\footnote{\url{https://vision.middlebury.edu/stereo/data/scenes2021/}}. This data collection consists of 24 indoor stereo datasets captured using a mobile device (Apple iPod touch 6G) mounted on a robotic arm, enabling acquisition of ground truth disparities via structured lighting. Spanning 11 distinct scenes imaged from 1-3 viewpoints under varying illuminations and exposures, including flash, ambient light, and device torch lighting, each dataset provides two $1920 \times 1080$ resolution views organized into directories containing multiple illumination/exposure variants alongside calibration data and ground truth disparity maps.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The Booster Dataset
% CVPR, 2022
% Open Challenges in Deep Stereo: The Booster Dataset
% https://openaccess.thecvf.com/content/CVPR2022/papers/Ramirez_Open_Challenges_in_Deep_Stereo_The_Booster_Dataset_CVPR_2022_paper.pdf
% https://cvlab-unibo.github.io/booster-web/
\textbf{Booster} \cite{Ramirez_2022_CVPR}\footnote{\url{https://cvlab-unibo.github.io/booster-web/}}. This work introduces a novel high-resolution stereo dataset targeting the open challenges of non-Lambertian surfaces and high-resolution stereo matching. The dataset consists of 419 high-resolution (12 Mpx) stereo image pairs, as well as 419 unbalanced pairs with a 12 Mpx left image and 1.1 Mpx right image, collected across 64 different indoor scenes. The scenes contain a variety of specular and transparent surfaces, which are carefully annotated with dense ground-truth disparities using a novel deep space-time stereo framework. This framework leverages a pre-trained deep stereo network to accumulate cost volumes from multiple textured stereo pairs, enabling accurate sub-pixel disparity labels even for the challenging non-Lambertian regions. In addition to the ground-truth disparities, it provides manually annotated material segmentation masks to facilitate analysis of network performance on different surface types. The dataset is divided into 228 training and 191 test samples, where the test ground truth disparities are withheld, providing a challenging benchmark to encourage further research on these open problems in stereo matching. The dataset is accompanied by an online evaluation benchmark for assessing stereo methods.%\cite{ramirez2023booster}, \cite{ramirez2023ntire}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Holopix50k
% CVPR, 2020
% Holopix50k: A large-scale in-the-wild stereo image dataset
% https://leiainc.github.io/holopix50k/
% https://arxiv.org/abs/2003.11172
\textbf{Holopix50k}\cite{hua2020holopix50k}\footnote{\url{https://github.com/leiainc/holopix50k}}. Holopix50k is an in-the-wild stereo dataset comprising 49,368 image pairs captured by users of the Holopix mobile social platform, covering a wide variety of realistic scenarios in mobile photography. The images have an average resolution of 0.74 (±0.30) Mpx and were collected from the first Lightfield-enabled social media application. The dataset underwent post-processing steps to ensure high-quality stereo pairs, including removing vertical disparity and disparity-based filtering. However, Holopix50k contains only stereo RGB images without any ground truth disparity, making it suitable for self-supervised training of stereo networks. Moreover, due to the lack of ground truth disparity, Holopix50k is not typically used as a benchmark for evaluating stereo vision algorithms.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% InStereo2K
% Science China Information Sciences, 2020
% Instereo2k: a large real dataset for stereo matching in indoor scenes
% https://link.springer.com/article/10.1007/s11432-019-2803-x
% https://github.com/YuhuaXu/StereoDataset
\textbf{InStereo2K}\cite{bao2020instereo2k}\footnote{\url{https://github.com/YuhuaXu/StereoDataset}}. The InStereo2K dataset is a large-scale stereo dataset designed for indoor scenes, containing 2050 pairs of stereo images with highly accurate disparity maps obtained using a structured light system. The dataset is split into a training set of 2000 image pairs and a test set of 50 image pairs, with a resolution of $1080 \times 860$ pixels. InStereo2K covers a wide range of indoor scenes, including offices, classrooms, bedrooms, living rooms, and dormitories. The structured light system used to generate the dataset consists of two color cameras with a resolution of $1280 \times 960$ pixels and a projector with a resolution of $1024 \times 768$ pixels.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{Multimodal Stereo Datasets}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% CATS
% CVPR, 2017
% CATS: A Color and Thermal Stereo Benchmark
% https://openaccess.thecvf.com/content_cvpr_2017/papers/Treible_CATS_A_Color_CVPR_2017_paper.pdf
\textbf{CATS}\cite{Treible_2017_CVPR}\footnote{\url{https://bigdatavision.org/CAT/download.html}}. The Color and Thermal Stereo (CATS) dataset is a large-scale benchmark consisting of approximately 1400 images captured by a sensor platform with two visible-band cameras at a resolution of $1280 \times 960$ pixels, two long wave infrared (LWIR) thermal cameras at a resolution of $640 \times 480$ pixels, and a LiDAR for high-accuracy (<2mm) ground truth. The dataset features 100 indoor and 80 outdoor cluttered scenes with diverse objects under various lighting and environmental conditions. CATS provides rectified stereo pairs in color, thermal, and cross-modality configurations, along with corresponding ground truth disparity maps generated by projecting the LiDAR data onto the images using a novel semi-automatic calibration method. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% MVSEC
% RAL 2018
% The Multivehicle Stereo Event Camera Dataset: An Event Camera Dataset for 3D Perception
% https://arxiv.org/abs/1801.10202
% https://daniilidis-group.github.io/mvsec/
\textbf{MVSEC}\cite{mvsec}\footnote{\url{https://daniilidis-group.github.io/mvsec/}}. The Multi Vehicle Stereo Event Camera dataset (MVSEC) collects data from both indoor and outdoor environments with event cameras. Specifically, a 10cm-baseline stereo camera made with DAVIS 346B sensors collects event frames at 346$\times$260 resolution, together with a grayscale stereo camera mounting Aptina MT9V034 sensors working at $752\times480$ resolution, 
a Velodyne Puck LITE (16-lines) to collect sparse depth data, an IMU, motion capture, and GPS. This sensor suite allows for extracting accurate ground truth pose and disparity maps -- the latter obtained by accumulating LiDAR point clouds according to a LiDAR odometry pipeline (LOAM \cite{zhang2014loam}).
Sequences are collected in a mixture of indoor and outdoor environments from different vehicles: 6 from a hexacopter, 5 from a car, one from a motorcycle, and 2 when the camera is handheld, both during day and night.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% DSEC
% RAL, 2021
% {DSEC}: A Stereo Event Camera Dataset for Driving Scenarios
% https://rpg.ifi.uzh.ch/docs/RAL21_DSEC.pdf
% https://github.com/uzh-rpg/DSEC
% https://dsec.ifi.uzh.ch/
\textbf{DSEC} \cite{gehrig2021dsec}\footnote{\url{https://dsec.ifi.uzh.ch/}}. The DSEC (Driving Stereo Event Camera) dataset is designed to address the challenges faced by standard cameras in adverse lighting conditions such as night, sunrise and sunset.  It provides a rich set of sensory data, including a wide-baseline stereo setup with two color frame cameras ($1440 \times 1080$ resolution, 51 cm baseline) and two high-resolution monochrome event cameras ($640 \times 480$ resolution, 60 cm baseline), which offer unique advantages like high temporal resolution, high dynamic range, reduced motion blur, and low latency. The dataset contains 53 sequences collected in various illumination conditions and environments in Switzerland, totaling over 4 TB of raw data, and also includes LiDAR data, RTK GPS measurements, accurate time synchronization, and calibration between sensors. DSEC provides ground truth disparity and incorporates sequences with challenging illumination conditions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% M3ED
% CVPR, 2023
% M3ed: Multi-robot, multi-sensor, multi-environment event dataset
% https://openaccess.thecvf.com/content/CVPR2023W/EventVision/papers/Chaney_M3ED_Multi-Robot_Multi-Sensor_Multi-Environment_Event_Dataset_CVPRW_2023_paper.pdf
% https://m3ed.io/
\textbf{M3ED} \cite{Chaney_2023_CVPR}\footnote{\url{https://m3ed.io/}}. This dataset provides 57 indoor/outdoor scenes collected with a compact multi-sensor block mounted on three different vehicles -- a car, a UAV, and a quadruped robot.
The event stereo camera mounts Prophesee Gen 4 sensors, capturing frames at $1280\times720$ resolution with a 12cm baseline, accompanied by a color stereo camera mounding OVC 3b sensors working at $1280\times800$ resolution with an equivalent baseline.
A 64-line Ouster OS1-64U LiDAR is used to generate semi-dense ground-truth disparity maps, by accumulating single scans through LiDAR odometry (FasterLIO \cite{fasterlio}). In total, M3ED provides about 3TB of raw and processed data.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Gated Stereo
% CVPR, 2023
% Gated Stereo: Joint Depth Estimation from Gated and Wide-Baseline Active Stereo Cues
% https://openaccess.thecvf.com/content/CVPR2023/papers/Walz_Gated_Stereo_Joint_Depth_Estimation_From_Gated_and_Wide-Baseline_Active_CVPR_2023_paper.pdf
% https://light.princeton.edu/gatedstereo/
\textbf{Gated Stereo} \cite{walz2023gated}\footnote{\url{https://light.princeton.edu/gatedstereo/}}.  Gated Stereo is a long-range dataset that was captured to facilitate training and evaluation of depth estimation methods that leverage gated imaging and stereo cues. Gated imaging enables robust long-range depth measurement by using active illumination and measuring time-of-flight, overcoming limitations of passive techniques. The dataset was acquired by driving over 1000 km in Germany with a sensor suite comprising a long-range LiDAR, an RGB stereo camera, and a synchronized NIR gated stereo camera. The gated camera captures $1280 \times 720$ resolution images at 120 Hz, providing 3 gated slices and 2 ambient exposures enabled by active VCSEL illumination. The RGB stereo camera provides $1920 \times 1080$ images at 30 Hz. The dataset contains over 107,000 samples captured across day, night, and varying weather conditions. After being curated for scenario diversity, it is divided into 54,320 samples for training, 728 for validation, and 2,463 for testing.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% RGB-MS
% CVPR, 2022
% RGB-Multispectral Matching: Dataset, Learning Methodology, Evaluation
% https://openaccess.thecvf.com/content/CVPR2022/papers/Tosi_RGB-Multispectral_Matching_Dataset_Learning_Methodology_Evaluation_CVPR_2022_paper.pdf
% https://cvlab-unibo.github.io/rgb-ms-web/
\textbf{RGB-MS}\cite{tosi2022rgb}\footnote{\url{https://cvlab-unibo.github.io/rgb-ms-web/}}. The RGB-MS dataset tackles the novel challenge of registering synchronized RGB and multi-spectral (MS) images with vastly different resolutions via stereo matching. It comprises 34 indoor RGB-MS image pairs from 13 scenes, with 12.4MP RGB images paired with 2.2MP 10-band MS images and annotated with high-resolution semi-dense ground truth disparities. These were generated using an additional 12.2MP RGB camera during acquisition - static scenes perturbed with patterns enabled robust disparity estimation from active RGB stereo pairs via cost volume integration, semi-global matching, outlier removal, and warping to the RGB-MS views. 11K unlabeled RGB-RGB-MS triplets are also provided in both indoor and outdoor environments. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% MS^2
% CVPR 2023
% Deep Depth Estimation From Thermal Image
% https://openaccess.thecvf.com/content/CVPR2023/papers/Shin_Deep_Depth_Estimation_From_Thermal_Image_CVPR_2023_paper.pdf
% https://sites.google.com/view/multi-spectral-stereo-dataset
$\mathbf{MS^2}$\cite{Shin_2023_CVPR}\footnote{\url{https://sites.google.com/view/multi-spectral-stereo-dataset}}. The Multi-Spectral Stereo ($\mathbf{MS^2}$) dataset is a large-scale collection of synchronized multi-modal data captured for autonomous driving, comprising around 195K data pairs of stereo RGB images ($2448 \times 2048$ resolution, 15fps), stereo near-infrared (NIR) images ($1280 \times 720$ resolution, 15fps), stereo long-wave infrared (thermal) images ($640 \times 512$ resolution, 30fps), stereo LiDAR point clouds (10fps), and GNSS/IMU information. The data was acquired across diverse environments like cities, residential areas, roads, and campuses, under varying conditions including daytime, nighttime, cloudy, and rainy weather. The thermal stereo images are provided along with semi-dense ground truth depth maps generated by accumulating successive LiDAR sweeps and utilizing interpolated odometry. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% RPS
% ICCV, 2023
% DPS-Net: Deep Polarimetric Stereo Depth Estimation
% https://openaccess.thecvf.com/content/ICCV2023/papers/Tian_DPS-Net_Deep_Polarimetric_Stereo_Depth_Estimation_ICCV_2023_paper.pdf
% https://github.com/Ethereal-Tian/DPS-Net
$\mathbf{RPS}$\cite{Tian_2023_ICCV}\footnote{\url{https://github.com/Ethereal-Tian/DPS-Net}}. The Real Polarimetric Stereo dataset (RPS) is a collection of 1,300 stereo pairs -- 1,000 of which have been collected indoors, while the remaining 300 are in outdoor environments. Two Lucid PHX050S-Q polarization cameras have been used
to capture stereo polarization images at 1280$\times$960 resolution, paired with an RGB-D camera for collecting ground-truth depth.
Each polarization camera in the pair captures four polarization images, with different polarizer angles in a single shot.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Synthetic}

We now introduce more datasets obtained through graphic engines, allowing for generating vast amounts of stereo images and dense ground truth disparities with little effort. Fig. \ref{fig:synth_dataset} shows an overview of same samples taken from these datasets.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% HS-VS
% CVPR, 2019
% Hierarchical deep stereo matching on high-resolution image
% https://arxiv.org/pdf/1912.06704.pdf
% https://github.com/gengshan-y/high-res-stereo?tab=readme-ov-file
\textbf{HR-VS}\cite{Yang_2019_CVPR}\footnote{\url{https://github.com/gengshan-y/high-res-stereo?tab=readme-ov-file}}. The High-res Virtual Stereo (HR-VS) dataset, presented in \cite{Yang_2019_CVPR} along with the HSMNet architecture, is a synthetic high-resolution stereo dataset generated using the Carla simulator \cite{dosovitskiy2017carla}. It contains 780 pairs of stereo images at $2056 \times 2464$ pixel resolution collected under 4 weather conditions in Town01, with a camera baseline of 0.54m. The dataset mimics real-world driving scenarios by limiting the disparity range to [9.66, 768] pixels and the depth range to [2.52, 200] meters, making it suitable for training high-resolution stereo matching algorithms for autonomous driving and urban scene understanding.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Virtual kitti 2
% arXiv, 2020
% Virtual kitti 2
% https://arxiv.org/pdf/2001.10773
% https://europe.naverlabs.com/Research/Computer-Vision/Proxy-Virtual-Worlds/
\textbf{Virtual KITTI 2}\cite{cabon2020virtual}\footnote{\url{https://europe.naverlabs.com/Research/Computer-Vision/Proxy-Virtual-Worlds/}} Building upon its predecessor, Virtual KITTI~\cite{Gaidon_CVPR_2016}, this dataset offers photo-realistic renderings of driving scenarios generated using the Unity game engine. The dataset comprises 5 image sequences, each a clone of a real-world sequence from the KITTI tracking benchmark, with a resolution of $1242 \times 375$ pixels. What sets Virtual KITTI 2 apart is its diverse set of renditions for each sequence, including variations in weather conditions like fog and rain, as well as modifications to the camera configuration, such as rotations of $15^\circ$ and $30^\circ$. In addition to RGB images, the dataset provides ground truth data for depth, optical flow, scene flow, instance segmentation, and semantic segmentation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Tartanair
% IROS, 2020
% Tartanair: A dataset to push the limits of visual slam
% https://ieeexplore.ieee.org/document/9341801?denied=
% https://theairlab.org/tartanair-dataset/shorter 
\textbf{TartanAir}\cite{wang2020tartanair}\footnote{\url{https://theairlab.org/tartanair-dataset/}}. The TartanAir dataset is a large-scale, challenging dataset designed for robot navigation tasks, with a special focus on stereo vision and SLAM-related problems. It provides synchronized stereo RGB images across 1037 long motion sequences in 30 diverse environments, covering structured urban and indoor scenes as well as unstructured natural environments, resulting in over 1 million frames. Collected in photo-realistic simulation using the Unreal Engine and AirSim plugin, the dataset also includes depth images, segmentation labels, camera poses, occupancy grid maps, optical flow, stereo disparity, and simulated LiDAR measurements. TartanAir covers a wide range of motion patterns and includes challenging scenes with dynamic lighting, low illumination, adverse weather, and dynamic objects, aiming to bridge the gap between simulation and real-world performance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% UnrealStereo4K
% CVPR, 2021
% SMD-Nets: Stereo Mixture Density Networks
% http://www.cvlibs.net/publications/Tosi2021CVPR.pdf
% https://github.com/fabiotosi92/SMD-Nets
\textbf{UnrealStereo4K} \cite{Tosi2021CVPR_SMD} \footnote{\url{https://github.com/fabiotosi92/SMD-Nets}}. The UnrealStereo4K dataset is a large-scale synthetic stereo dataset created using the Unreal Engine and the open-source plugin UnrealCV. It consists of 8 scenes, including both indoor and outdoor environments, with a total of 8,000 stereo pairs at $3840 \times 2160$px resolution. The dataset is divided into 7,720 training pairs, 80 validation pairs, and 200 in-domain test pairs. An additional 200 out-of-domain test pairs from an unseen scene are provided to evaluate the generalization ability of stereo matching methods. The baseline is set to 20cm for indoor environments and 50cm for outdoor environments. The camera poses are randomly sampled, and invalid camera poses and stereo pairs are filtered out based on minimum depth, image intensity, and disparity map gradient criteria to ensure non-trivial geometry structure in the dataset.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% IRS
% ICME, 2021
% IRS: A large naturalistic indoor robotics stereo dataset to train deep models for disparity and surface normal estimation
% https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9428423&casa_token=wdItdcnJ3QkAAAAA:OZDqHpMb0LlKp_t_unpp8aZWh0dvRai0KkZAtdI_jvioFMqjv3goGrR3AIjmObzMjRmE_7k
% https://github.com/HKBU-HPML/IRS
\textbf{IRS} \cite{wang2021irs}\footnote{\url{https://github.com/HKBU-HPML/IRS}}. The IRS (Indoor Robotics Stereo) dataset is a large-scale synthetic stereo dataset designed for indoor robotics applications, containing over 100,000 stereo image pairs (84,946 for training and 15,079 for testing) with a resolution of $960 \times 540$ pixels. The dataset covers four indoor scene types (home, office, restaurant, and store) and 70 different scene layouts, with more than 2,091 identical furniture objects of various types placed within the constructed spaces. IRS provides high-quality and dense ground truth labels for surface normal and disparity maps, which are crucial for training deep learning models. The dataset is generated using a customized version of Unreal Engine 4 with originally implemented plug-ins, ensuring that the rendered images closely resemble real-world scenes in terms of material texture, light reflection and transmission, shadows, bloom, and lens flare. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% CREStereo
% CVPR, 2022
% Practical stereo matching via cascaded recurrent network with adaptive correlation
% https://openaccess.thecvf.com/content/CVPR2022/papers/Li_Practical_Stereo_Matching_via_Cascaded_Recurrent_Network_With_Adaptive_Correlation_CVPR_2022_paper.pdf
% https://github.com/megvii-research/CREStereo
\textbf{CREStereo} \cite{li2022practical_CREStereo}\footnote{\url{https://github.com/megvii-research/CREStereo}}.
In the paper introducing the CREStereo architecture, a synthetic dataset for training stereo matching algorithms is also proposed. This dataset, generated using Blender, includes left-right image pairs and corresponding dense disparity maps. The dataset scenes feature a variety of object shapes sourced from ShapeNet and custom models with complex characteristics such as holes and open-work structures. Additionally, the dataset incorporates complex lighting environments with random colors and luminance, using real-world images as textures for objects and backgrounds. To ensure a wide range of disparity, objects are randomly positioned within the virtual cameras' field of view, with varying distances and scales.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% SimStereo
% NeurIPS, 2022
% Active-Passive SimStereo – Benchmarking the Cross-Generalization Capabilities of Deep Learning-based Stereo Methods
% https://proceedings.neurips.cc/paper_files/paper/2022/file/bc3a68a20e5c8ba5cbefc1ecf74bfaaa-Paper-Datasets_and_Benchmarks.pdf
% https://ieee-dataport.org/open-access/active-passive-simstereo
\textbf{SimStereo} \cite{jospin2022active_SimStereo}\footnote{\url{https://ieee-dataport.org/open-access/active-passive-simstereo}}. The Active-Passive SimStereo dataset contains 515 computer-generated image pairs with a resolution of $640 \times 480$ pixels, rendered using a physically-based rendering engine. This ensures that the images closely resemble real-world scenes in terms of material texture, light reflection, transmission, shadows, bloom, and lens flare. The dataset is split into a training set of 412 image pairs and a test set of 103 image pairs, covering various shapes, depth ranges, and styles. The test set includes realistic scenes and abstract compositions to effectively benchmark the performance of stereo vision models. SimStereo provides both active and passive frames for each scene, allowing for a direct comparison of the relative performance of algorithms in both scenarios.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Spring
% CVPR, 2023
% Spring: A High-Resolution High-Detail Dataset and Benchmark for Scene Flow, Optical Flow and Stereo
% https://openaccess.thecvf.com/content/CVPR2023/html/Mehl_Spring_A_High-Resolution_High-Detail_Dataset_and_Benchmark_for_Scene_Flow_CVPR_2023_paper.html
% http://spring-benchmark.org
\textbf{Spring} \cite{Mehl2023_Spring}\footnote{\url{http://spring-benchmark.org}}. The Spring dataset introduces a large, high-resolution, high-detail, synthetic benchmark for scene flow, optical flow, and stereo estimation. Based on rendered scenes from the open-source Blender movie ``Spring", it provides 6,000 stereo image pairs from 47 sequences at $1920 \times 1080$ resolution, along with 12,000 ground truth frames for stereo and 23,812 ground truth frames for motion - 60x more than KITTI 2015 and 15x more than MPI Sintel. To adequately assess fine details, the dataset uses a novel evaluation methodology based on super-resolved ($3840 \times 2160$px) ground truth, and provides focused evaluations on different image regions including high-detail, unmatched, non-rigid, sky, and large-displacement areas. The dataset is accompanied by a public benchmark website to upload, analyze and compare novel methods.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Dynamic Replica
% CVPR 2023
% DynamicStereo: Consistent Dynamic Depth From Stereo Videos
% https://openaccess.thecvf.com/content/CVPR2023/papers/Karaev_DynamicStereo_Consistent_Dynamic_Depth_From_Stereo_Videos_CVPR_2023_paper.pdf
% https://dynamic-stereo.github.io/
\textbf{Dynamic Replica}\cite{Karaev_2023_CVPR}\footnote{\url{https://dynamic-stereo.github.io/}}. Dynamic Replica is a synthetic stereo video dataset featuring 524 videos of animated humans and animals in everyday scenes, designed for training temporally consistent models. The dataset includes 484 training videos, 20 validation videos (both 10 seconds long with 300 frames each), and 20 test videos (30 seconds long), all rendered at $1280 \times 720$ resolution. The dataset is based on Facebook Replica reconstructions, using 375 3D human scans and 13 animal categories, with randomized camera baselines between 4cm and 30cm in the training subset. All samples contain ground-truth depth maps, optical flow, segmentation masks, and camera parameters for both stereo views.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> chapters/8_metrics.tex <==
\subsection{Evaluation Metrics}
\label{sec:metrics}

The evaluation of stereo methods is typically performed by comparing the estimated disparity maps against ground truth data using several metrics. A widely adopted metric is the End-Point Error (EPE)$\downarrow$, defined as:

\begin{equation}
    \text{EPE} = \frac{1}{N}\sum_{p}|D_p - D_p^{gt}|
\end{equation}
where $D_p$ and $D_p^{gt}$ are the predicted and ground truth disparity values for pixel $p$, respectively, and $N$ is the total number of pixels. The EPE calculates the average absolute difference between the predicted and ground truth disparity values across all pixels.
Optionally, the Root Mean Squared Error (RMSE) is also taken into account in some benchmarks, such as Middlebury v3 and Booster:

\begin{equation}
    \text{RMSE} = \sqrt{\frac{1}{N}\sum_{p}(|)D_p - D_p^{gt})^2}
\end{equation}

Moreover, existing benchmarks commonly report the bad-$\tau$ error$\downarrow$, defined as the percentage of pixels whose disparity estimation deviates by more than $\tau$ pixels from the ground truth:

\begin{equation}
\text{bad-}\tau = \frac{1}{N}\sum_{p} \delta(|D_p - D_p^{gt}| > \tau)
\end{equation}
where $\delta$ is the indicator function that returns 1 if the condition is true, and 0 otherwise. 
On the KITTI 2015 benchmark, a variant of the bad metric, the D1 error, is adopted:

\begin{equation}
\begin{split}
D1 = \frac{1}{N}\sum_{p} \delta( &|D_p - D_p^{gt}| > 3 \land \\ &|D_p - D_p^{gt}| > 0.05\cdot D_p^{gt}) 
\end{split}
\end{equation}
considering as outliers those disparities whose error surpasses 3 pixels and 5\% of the ground-truth value.

==> images/nerf-stereo_vs_LSSI_depth.tex <==
\begin{figure}[t]
\centering
\renewcommand{\tabcolsep}{1pt}
\begin{tabular}{ccc}
\includegraphics[width=0.16\textwidth]{./images/0150.jpg} &
\includegraphics[width=0.16\textwidth]{./images/midas/0150_spectral.jpg} & 
\includegraphics[width=0.16\textwidth]{./images/nerf/0150_spectral.jpg}  \\
\includegraphics[width=0.16\textwidth]{./images/0156.jpg} &
\includegraphics[width=0.16\textwidth]{./images/midas/0156_spectral.jpg} & 
\includegraphics[width=0.16\textwidth]{./images/nerf/0156_spectral.jpg}  \\
\includegraphics[width=0.16\textwidth]{./images/0163.jpg} &
\includegraphics[width=0.16\textwidth]{./images/midas/0163_spectral.jpg} & 
\includegraphics[width=0.16\textwidth]{./images/nerf/0163_spectral.jpg}  \\
\end{tabular}
\vspace{-0.3cm}
\caption{\textbf{LLSI vs NS-Stereo Labels.} From left to right: RGB images from scenes in the NS-Stereo dataset and corresponding depth maps by MidAs \cite{Ranftl2022} and Instant-NGP \cite{muller2022instant}.}
\label{fig:image_collection11}
\end{figure}

==> tables/dsec.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
\rowcolors{2}{salmon}{white}
\scalebox{0.85}{
\begin{tabular}{ll cccc}

\Xhline{2pt}
\multirow{2}{*}{Method}  & \multirow{2}{*}{Venue} & \multicolumn{4}{c}{DSEC}\\
\cmidrule(lr){3-6}
& &  1PE $\downarrow$  & 2PE $\downarrow$ & MAE $\downarrow$ & RMSE $\downarrow$ \\

\toprule

\hyperlink{EI-Stereo}{\textcolor{magenta}{EI-Stereo}}~\cite{mostafavi2021event_intensity}         & ICCV 2021    & 5.814 & 1.055 & 0.396 & 0.906 \\
\hyperlink{SE-CFF}{\textcolor{magenta}{SE-CFF}}~\cite{Nam_2022_CVPR_CFF}         & CVPR 2022    & 9.583 & 2.620 & 0.519 & 1.231 \\
\hyperlink{DTC-SPADE}{\textcolor{magenta}{DTC-SPADE}}~\cite{Zhang_2022_CVPR_DTC_SPADE}         & CVPR 2022    & 9.277 & 2.416 & 0.527 & 1.291 \\
\bottomrule

\end{tabular}
}
\caption{\textbf{DSEC Online Benchmark}}
\label{table:dsec}
\end{table}

==> tables/zero_shot_generalization.tex <==
\begin{table*}[t]
\centering
    \scalebox{0.8}{
            \begin{tabular}{cc}
                \begin{tabular}{c}
                 \\ \\ \\ \\ \\ \\ \\ \\ \\ \\ (A) \\ \\ \\ \\ \\ \\ \\ \\ \\ (B) \\ \\ \\ \\ \\ \\ (C) \\ \\ (D) \\
                \end{tabular}\kern-1.6em  
            &
            \renewcommand{\tabcolsep}{12pt}
            \rowcolors{2}{salmon}{white}
            \begin{tabular}{lc|rr|rrrrrr|rr}
                \Xhline{2pt}
                & & \multicolumn{2}{c|}{KITTI-15} & \multicolumn{6}{c|}{Midd-T} & \multicolumn{2}{c}{ETH3D} \\
                Method & &  \multicolumn{2}{c|}{($>3$px)} & \multicolumn{2}{c}{F ($>2$px) } & \multicolumn{2}{c}{H ($>2$px)} & \multicolumn{2}{c|}{Q ($>2$px)} & \multicolumn{2}{c}{($>1$px)} \\
                \hline
                & & All & Noc & All & Noc & All & Noc & All & Noc & All & Noc \\
                \hline
                Training Set & \multicolumn{10}{c}{SceneFlow with GT} \\
                \hline         
                \rowcolor{white}
                GANet \cite{zhang2019ga}                      & & 10.46 & 10.15 & 45.36 & 40.80 & 26.75 & 21.8 & 15.52 & 11.49 & 8.68 & 7.75 \\
                DSMNet \cite{zhang2019domaininvariant_DSM}        & & 5.50 & 5.19 & 29.95 & 24.79 & 16.88 & 12.03 & 13.75 & 9.44 & 12.52 & 11.62 \\
                CFNet \cite{shen2021cfnet}                    & & 6.01 & 5.94 & 29.12 & 24.15 & 20.11 & 15.84 & 13.77 & 10.32 & 5.77 & 5.32 \\
                \rowcolor{white}
                MS-GCNet \cite{cai2020matchingspace}          & * & 6.21 & - & - & - & - & 18.52 & - & - & - & 8.84 \\
                \cdashline{3-12}
                RAFT-Stereo \cite{lipson2021raft}             & * & 5.74 & - & 18.33 & - & 12.59 & - & 9.36 & - & 3.28 & - \\
                RAFT-Stereo \cite{lipson2021raft}             & \textdaggerdbl &  5.45 & 5.21 & \bfseries \silver{18.20} & \bfseries \silver{14.19} & \bfseries \silver{11.19} & \bfseries \silver{8.09} & \bfseries \silver{9.31} & \bfseries \silver{6.56} & \bfseries \gold{2.59} & \bfseries \silver{2.24} \\
                \cdashline{3-12}
                SGM + NDR \cite{aleotti2021neural}            & &  5.41 & 5.12 & 27.27 & 21.09 & 17.70 & 13.51 & 11.75 &  7.93 & \bronze{5.20} & \bronze{4.78} \\         
                STTR \cite{Li_2021_ICCV_STTR}                  & &  8.31 & 6.73 & 38.10 & 30.74 & 26.39 & 18.17 & 15.91 & 8.51 & 20.49 & 19.06\\ % MASSIMA RISOLUZIONE MIDDLEBURY: HALF * 0.85
                CEST \cite{guo2022context_CEST}                    & &  7.61 & 6.13 & 27.44 & 19.53 & 19.89 & 11.82 & 14.71 & 7.56 & 10.99 & 9.78\\ % MASSIMA RISOLUZIONE MIDDLEBURY: HALF
                FC-GANet \cite{Zhang_2022_CVPR_FCStereo}           & * & 5.3x & - & - & - & - & 10.2x & - & 7.8x & 5.8x & - \\
                ITSA-GWCNet \cite{Chuah_2022_CVPR_ITSA}              & &  5.60 & 5.39 & 29.46 & 25.18 & 19.38 & 15.95 & 14.36 & 10.76 & 7.43 & 7.12 \\
                ITSA-CFNet \cite{Chuah_2022_CVPR_ITSA}               & &  \bfseries \gold{4.96} & \bfseries \gold{4.76} & 26.38 & 21.41 & 18.01 & 14.00 & 13.32 & 9.73 & 5.40 & 5.14 \\       
                CREStereo \cite{li2022practical_CREStereo}              & \textdaggerdbl & 5.79 & 5.40 & 34.78 & 30.52 & 17.57 & 13.87 & 12.88 & 8.85 & 8.98  & 8.14 \\
                \hline
                PSMNet \cite{chang2018pyramid_PSMNet}                 & \textdaggerdbl & 7.86 & 7.40 & 33.69 & 28.35 & 21.69 & 16.92 & 17.24 & 12.37 & 23.19 & 22.12 \\
                MS-PSMNet \cite{cai2020matchingspace}         & * &  7.76 & - & - & - & - & 19.81 & - & - & - & 16.84 \\
                Graft-PSMNet\cite{Liu_2022_CVPR_GraftNet}            & &  \bfseries 5.34 & \bfseries 5.02 & \bfseries 25.46 & \bfseries 19.28 & \bfseries 17.81 & \bfseries 13.46 & \bfseries 14.18 & \bfseries 9.21 & 11.42 & 10.69 \\
                FC-PSMNet \cite{Zhang_2022_CVPR_FCStereo}          & * & 5.8x & - & - & - & - & 15.1x & - &  9.3x & \bfseries 9.5x & - \\
                ITSA-PSMNet \cite{Chuah_2022_CVPR_ITSA}              & &  6.00 & 5.73 & 32.09 & 27.46 & 20.83 & 17.14 & 14.68 & 11.05 & 10.34 & \bfseries 9.77 \\   
                \hline

                Training Set & \multicolumn{10}{c}{Real-world data without GT} \\
                \hline 
                Reversing\cite{aleotti2020reversing}-PSMNet   & & $[4.09]$ & $[3.88]$ & 38.23 & 30.00 & 26.45 & 20.91 & 20.55 & 15.08 & 9.00 & 8.23 \\
                LSSI\cite{watson2020learning_LSSI}-PSMNet             & & \bronze{5.18} & \bronze{4.91} & 26.42 & 21.38 & 17.56 & 13.45 & 12.07 & 9.09 & \bfseries 8.17 & \bfseries 7.44 \\
                NS-PSMNet \cite{Tosi_2023_CVPR}                                     & & \bfseries \silver{5.05} & \bfseries \silver{4.80} & \bfseries \bronze{20.60} & \bfseries \bronze{15.83} & \bfseries \bronze{12.91} & \bfseries \bronze{9.07} &  \bfseries \bronze{11.03} & \bfseries \bronze{7.15} & 11.69 & 11.00 \\
                \hline
                NS-RAFT-Stereo \cite{Tosi_2023_CVPR}                               & & 5.41 & 5.23 & \bfseries \gold{16.45} & \bfseries \gold{12.08} & \bfseries \gold{9.67} & \bfseries \gold{6.42} & \bfseries \gold{8.05} & \bfseries \gold{4.82} & \bfseries \silver{2.94} & \bfseries \gold{2.23} \\
    
                \hline
            \end{tabular}
            \end{tabular}
    }
    %\vspace{-0.3cm}
    \caption{\textbf{Zero-Shot Generalization Benchmark.} We test all models using authors' weights. Exceptions: $*$ numbers from the original paper; \textdaggerdbl{} retrained model.
    Best results per macro-block in \textbf{bold}. We also highlight \gold{\textbf{first}}, \silver{\textbf{second}} and \bronze{\textbf{third}} absolute bests. For RAFT-Stereo (in dashed lines) only the best between $*$ and \textdaggerdbl{} is kept for rankings. $[\kern.2em]$ means trained on the same domain, thus ignored for rankings. 
    }\vspace{-0.3cm}
\label{tab:zero}
\end{table*} % from NS-Supervised
